Causal Scene BERT: Improving object detection by searching for challenging groups of data

Modern computer vision applications rely on learning-based perception modules parameterized with neural networks for tasks like object detection. These modules frequently have low expected error overall but high error on atypical groups of data due to biases inherent in the training process. In building autonomous vehicles (AV), this problem is an especially important challenge because their perception modules are crucial to the overall system performance. After identifying failures in AV, a human team will comb through the associated data to group perception failures that share common causes. More data from these groups is then collected and annotated before retraining the model to fix the issue. In other words, error groups are found and addressed in hindsight. Our main contribution is a pseudo-automatic method to discover such groups in foresight by performing causal interventions on simulated scenes. To keep our interventions on the data manifold, we utilize masked language models. We verify that the prioritized groups found via intervention are challenging for the object detector and show that retraining with data collected from these groups helps inordinately compared to adding more IID data. We also plan to release software to run interventions in simulated scenes, which we hope will benefit the causality community.

==> core/prior_versions/1_introduction.tex <==
\section{Introduction}
\label{sec:intro}

% \karsten{Maybe add a little non-technical big picture motivation, I like this in papers. ``AV systems and machine learning and perception systems more generally are becoming parts of our daily lives...''}

% \orl{I would consider ordering a bit differently: (1) motivation (as-is) (2) setup (limit to simulation) (3) saying that naive addition of iid doesn't help and we need modes. (4) finding these modes is hard and we need a more efficient way to do it. (enters the MLM)}


Our guiding motivation in this paper is to understand where a detection module has poor performance \textit{before} it enters production. We focus on a realistic setting -- autonomous vehicles (AV). These systems are becoming more apparent in our lives as they enter mainstream. It is vital that this module is extremely capable, however biases in the training process such as in the data distribution, the chosen architecture, or the hyperparameters will lead to the model having atypical groups of data where the error is much higher than what it is in expectation over the full dataset. These gaps in its scene understanding lead to faulty operation, disengagements, and emergency consequences, and we would prefer that they be identified before deployment. We focus in this work on semantically meaningful groups such as specific weather patterns, vehicle types, and vehicle positioning. These are high priority problems to the community because finding challenging groups 
% parts of the data distribution 
% \karsten{We talk about AV stuff and detection, now we switch to very abstract language, i.e. data distribution. Would it be better to just refer to challenging scenes here?} 
in advance informs efficient data acquisition, in turn improving the robustness and safety of AV systems. However, na\"ively searching for them is difficult because the search space is so large. We are proposing a sophisticated approach to do this inspired by recent advances in masked language models~\cite{devlin2019bert} (MLM) and AV simulation frameworks, specifically CARLA~\cite{Dosovitskiy17}.

Those advances have granted us understanding of sequences such that we now reliably generate fluent language (see Section~\ref{sec:background}) and precisely control scene simulations. We leverage both of these by first encoding simulated scenes from synthetic data as flattened sequential scene graphs of symbolic tokens. We then mask out select tokens and use the trained MLM to infer new ones. This \textit{intervention}, e.g. changing the weather from sunny to dark, allows us to test causal interactions in a scene and see which are the most impactful.

% \karsten{We only point to the flexibility and control simulators offer us. Should we also say something about their realism regarding appearance (while still acknowledging sim2real issues)? I mean, if we couldn't place somewhat realistic 3D models, our work wouldn't be possible. I'm not sure, though.}
% \cinjon{I think you're asking to both say "hey these are closing the sim2real gap" and then also say "they aren't good enough yet and we dont actually do stuff irl int his paper. let's save that for the ending.}

\textbf{Our primary contribution is a method for taking such interventions on the data distribution using MLMs operating on scene graphs.} 
% \karsten{We highlight the MLM in this bold sentence here, but then only talk about it in the next paragraph. This isn't ideal. I would potentially skip the ``using...'' part and only in next paragraph start with something like ``We parametrize the interventions using a masked language ...'' etc.}
% \cinjon{I just introduced them earlier by adding in how the MLM advances helped us.}
We employ this procedure
% , along with machinery to understand the impact of these interventions, 
to find which groups in the data distribution 
are most challenging for the model
%, an example of which is the Diamondback bike asset, 
and confirm that the difficulty of these groups with respect to average precision (AP) aligns with our approach's predictions. We then show that adding independent and identically distributed (IID) data or more model capacity does not address the problem. Predictably, including data from the groups in training helps the model's performance on that group. Surprisingly, we find that including just one group in training helps every other group as well.

The MLM ensures that our interventions stay close to the true data distribution. 
%\karsten{This sounds unnecessarily abstract to me, maybe ``...interventions correspond to plausible and realistic scenes.''?}
%\cinjon{addressed offline}
This is critical, as we show via a comparison to random interventions that produces examples which are highly unlikely under the true data distribution. Consequently, using random interventions requires a much higher budget for data collection and model capacity than using the MLM interventions.

% We compare our proposed approach to a baseline where we randomly take an intervention instead of using the MLM. We would expect for random interventions to produce scene graphs which are highly unlikely under the actual data distribution; this impacts our budget for model capacity and data collection. On the other hand, a trained MLM will stay close to the distribution and alleviate this concern.

\textbf{Our second contribution is a toolbox for causal research.} We developed software that allows us to principally test questions of model capacity, dataset size, and dataset makeup. We did this in a simulated environment upon which we take causal interventions in a challenging and practical application setting. Beyond the AV community, we think this toolbox will benefit the causality community because the current state of the art~\cite{DBLP:journals/corr/abs-2012-07421} involves static datasets with low complexity tasks.
% \james{I think this looks great now!}
% \cinjon{:)}


% with labels that have naturally less inter-rater agreement than image recognition datasets. This is important because it is rare for actual real-world scenarios to have as high a label agreement as there is in popular image datasets (\cinjon{cite}). 

% Our final contributions are a dataset and an associated toolbox for creating similar datasets. The dataset was made by appealing to the gamescape (\cinjon{cite Open Ended Learning...}) associated with the hard examples. We started with the same initial training set and then appended successively more difficult blocks of data in which each block bested all previous models. We release this dataset as a challenging one for future models to face and additionally release all of the machinery that we wrote to make it. In addition to the AV world, we also think that this will be a strong contribution to the causal intervention world in that this machinery allows one to take principled interventions that remain on the data manifold.


==> core/prior_versions/3_background.tex <==
\section{Background}
\label{sec:background}

We train detection models on synthetic datasets from simulated AV environments, and take interventions using an MLM on scene graphs of those environments.


For the detection models, which operate on RGB images, we use the Detectron2 library~\cite{wu2019detectron2}. It provides a plethora of battle-tested architecture choices along with suggested training and testing configurations. We select six models: $18\textrm{C4}$, $18\textrm{FPN}$, $34\textrm{C4}$, $34\textrm{FPN}$, $50\textrm{C4}$, and $50\textrm{FPN}$. These are all common ResNet~\cite{he2015deep} architectures that include a litany of other attributes such as  Feature Pyramid Networks~\cite{lin2017feature}. See the Appendix for details. We create additional configurations that are 2x, 3x, 4x, and 5x wider versions of $50\textrm{FPN}$, exemplified by $50\textrm{FPN}2\textrm{x}$, for a total of ten tested model architectures. The $\textrm{C4}$ and $\textrm{FPN}$ mix allows us variation in model configuration, while the $18$, $34$, and $50$ layer counts and their width increases provide variation in capacity. We made minimal changes to the models to account for training on our dataset and with $4$ gpus instead of $8$. All models were trained for $90000$ steps (8-9 hours) without pre-training; none reached zero training loss. 

For data, we use the ubiquitous CARLA simulator and produce synthetic data from the preset Town03 or Town05 maps. Besides RGB images and COCO~\cite{lin2015microsoft} annotations for training the detectors, we also use \textit{scene graphs} to let the MLM semantically manipulate the scene. These are representations of an image in a deterministic tree structure with symbolic elements that each have symbolic or numeric attributes.
% \orl{maybe a quick example?}
We flatten the tree and use absolute positioning.

MLMs are trained by receiving sequences of discrete tokens, a small number of which are masked, and predicting what tokens should be in the masked positions. Through this process, they learn the data distribution~\cite{DBLP:journals/corr/abs-2009-10195,DBLP:journals/corr/abs-1902-04094} of those sequences. At inference, they are fed a sequence with a chosen token masked and replace the mask with their prediction. We use FairSeq~\cite{ott2019fairseq} and specifically the base MaskedLMModel transformer architecture\footnote{See masked\_lm.py\#L30 in the FairSeq library, commit hash 1bba712622b8ae4efb3eb793a8a40da386fe11d0} to train the MLM. We cannot use pre-trained models because our data is original, but instead train and validate on held out IID datasets of sequences converted from scene graphs (Section~\ref{sec:method}). These are converted to the FairSeq format before using the standard training pipeline.

For detection results on all charts, we report average precision (AP) over vehicles as returned by Detectron2. %The AP score is ubiquitous in detection.

% \karsten{I think in most papers the Background section is used for methodological background knowledge that is required to understand the novel contributions of the paper, which are then presented in the following Method section. Here, we use this section to discuss our implementation/experiment details instead (which models, data, etc.). I would usually provide this at the beginning of Experiments section and Appendix.}
% \cinjon{discussed offline}


==> core/prior_versions/4_method.tex <==
\section{Method}
\label{sec:method}


\begin{figure}[!t]
    \centering
    % \includegraphics[width=0.4\textwidth]{imgs/exp7/18_C4_1x.both.onlytwo.single.png}
    % \includegraphics[width=0.3\textwidth]{imgs/exp7/18_C4_1x.both.onlytwo.single.png}
    \setlength{\belowcaptionskip}{-10pt}
    \includegraphics[width=0.3\textwidth]{imgs/exp7/18_C4_1x.both.onlytwo.justbig..h3.750.png}
    \caption{After training models on any of four disjoint $10000$ IID subsets from CARLA's Town03 environment, they do well on the Town03 validation set and poorly on a validation set biased towards Diamondback bikes. This establishes that there is at least one challenging group for the model. Our method will now find other challenging groups.
    % \orl{Since this is kind of a teaser figure, i suggest we show not just the problem but also our solution.}
    }
    \label{fig:exp7-validate}
\end{figure}

% \orl{a general comment is that our Method section is too wordy and not formal enough. Why don't we start by setting up a formal notation and problem definition? As part of that, i'd specify what exactly we mean by ``scene graph'' which is an overloaded term. }

Figure~\ref{fig:exp7-validate} compares the performance of trained models on held-out data sampled from the training distribution and held-out data with increased occurrence of a challenging instance type, a brand of bikes called Diamondbacks. The performance gap between the sets is stark. We expected in advance that bikes would be difficult because they are underrepresented in the training distribution and are motivated to find similarly challenging groups with limited human involvement, especially groups that are not so easily hypothesized as the bikes.

One approach to doing this would be to iterate through the training set and gather examples for which the model $\phi$ gives poor results. Given a simulator R, if $x$ is a triplet of $(\textrm{scene graph}~G, \textrm{RGB image}~I, \textrm{label}~L)$, and $p_{\textrm{R}}(x)$ is the scene generation process, then we sample $(G, I, L) \sim p_{\textrm{R}}(x)$. To ascertain the model's ability on this example, we also need a per-example scoring function $f: (\phi, I, L) \rightarrow y$. Repeat this over the full training set to attain tuples $(G_i, y_i)$. 
% \james{I'm not sure that the extra notation here clarifies things. Shouldn't there be some time-dependent conditional information? Or otherwise, aren't you sampling stochastic processes $G^{(t)}, I^{(t)}, l^{(t)}$? I thought the AV perception modules were all time-dependent?}
% \cinjon{They aren't timedependnt - why did you think they were? Does something in htere suggest as much?}

We immediately run into a problem when trying to glean causal factors from this data because each $G_i$ has many scene constituents, such as the agents' attributes, the time of day, rain, etc, whose interactions scale combinatorially. The core issue is that we know the $y_i$ at too high of a level to parse which constituents were problematic.
% \james{is this accurate? Aren't there per-object bounding boxes?}, 
% \ak{agree with james, we could theoretically do more than a $y_i$ per image. But we would still not be able to tell causal factors} 
Even if we associate a score per ground truth bounding box, we still would not be able to disambiguate the cause because there are a multitude of reasons why a specific detection could fail that are a consequence of the interactions within a scene. Understanding those causes is important because it would help us in both finding more data that would patch the deficiency but also downstream in grokking whether we have sufficiently addressed the issue.

% \subsection{Causal interventions on simulated scenes}
\paragraph{Causal interventions on simulated scenes} We take inspiration from causal inference where interventions allow us to assess the causal links between the scene and the model's score. We change an aspect of a scene $G_i$, such as a rotation or location of a specific car, render this new scene $G_{i}^\prime$ as RGB image $I^\prime$, and then compute the $\delta = f(\phi, I^\prime, L^\prime) - f(\phi, I, L)$. If this $\delta$ is sufficiently negative (or positive), then the target (or original) attribute in the intervention is potentially problematic for $\phi$. We decide sufficiency by whether $|\delta| \ge \tau$, where $\tau > 0$ is a threshold parameter. After performing this procedure $N$ times and grouping by the intervention type, we attain an ordered list of challenging groups at the semantic level of specific rotations, car types, or weather patterns.

\paragraph{What determines the intervention?} Intervening randomly produces data that is unlikely under the true distribution, which makes it challenging to draw conclusions about the difficulty of the example with respect to its actual utility in improving our model. In other words, we would like for the model to be able to detect every semantic group ranging from out-of-distribution ones like flying cars to common ones like motorbikes in the dark. Given a computational budget, the latter is much higher priority than the former. Consequently, we should favor finding groups that have higher probability under the distribution and use a better technique than random interventions. This is especially true for a limited model capacity because learning to detect flying cars and other unrealistic low-priority scenarios will take capacity away from pressing needs; it is also true in practice because detection labeling is expensive and our budget for data outside of the simulator is never infinite.

With $p_{\textrm{R}}(x)$ as the generation process, $y$ our surrogate score, and $z$ a confounder that affects both $x$ and $y$, we need to draw a counterfactual $x^\prime$ that is independent of $z$. Sampling from $p_{\textrm{R}}(x)$ is challenging because retrieving the same scene again with just one change is difficult. Instead, we train a denoising autoencoder (DAE) to sample faithfully from $p_{\textrm{R}}(x)$~\cite{DBLP:journals/corr/abs-1305-6663,DBLP:journals/corr/abs-1905-12790,10.1145/1390156.1390294}. This sampling
% \ak{sampling counterfactuals from the data distribution -- just suggesting to spell it out again} 
is satisfied by using a masked language model (MLM) as our DAE~\cite{DBLP:journals/corr/abs-2009-10195,DBLP:journals/corr/abs-1902-04094}. 
% \karsten{Maybe rephrase this sentence: ``Considering our data structure, a masked language model (MLM) appears to be an appropriate choice for the DAE in our situation~\cite{...}.'' }

% We perform tahis with flattened scene graphs as sentences and believe we are the first to use this procedure for causal inference over scenes. 

The MLM is trained on flattened scene graphs where the discrete tokens are representations of weather, agent asset types, rotations, and locations (details below). These scenes were sampled from the same training distribution as that of the original detection module, albeit were not actually the same images. Figure~\ref{fig:scenegraphconversion} shows how, at inference time, we convert $G$ to a flat sequence $S$ and re-sample masked tokens to create counterfactual scenes. 
% \textbf{We believe we are the first to use this procedure for causal interventions over scenes.} 
Because the model was trained to a low perplexity on data drawn from the distribution, it faithfully samples from the original distribution $p_{\textrm{R}}(x)$. Because our model is not the exact distribution and errors will accumulate when applying many interventions sequentially, we intervene for just one categorical step, equivalent to a single node change in the scene graph.

% %%% Joan
% {\color{blue}what is the movitation to `discretize' the problem and recast it in terms of a `language'? Why not simply act directly on the attributed scene graph by modeling conditional distributions (conditnioning in all but one node, ie Gibbs sampling) and defining interventions directly as sampling from these conditional distributions? }
Observe that we could act directly on the scene graph and model the conditional distributions of a single node change. We would then use select changes via Gibbs sampling and define interventions as sampling from these conditional distributions. We choose to use discretization~\cite{oord2016wavenet,DBLP:journals/corr/EngelRRDESN17,razavi2019generating} and masked language models~\cite{dosovitskiy2021image,khan2021transformers} because of the recent and increasing success of these models in modeling the distribution, regardless of whether that distribution is naturally discrete such as in language.

\paragraph{Scene-sequence encoding} Encoding the scene graph language requires us to translate $G$ with continuous node attributes into discrete $S$. The first $10$ tokens correspond to weather attributes (cloudiness, precipitation, sun altitude angle, etc), the next $5$ are camera intrinsics, and the following $15$ represent the ego agent. After these $30$, we have a variable number of agents, each sequentially represented by $17$ tokens. The two extra tokens for the non-ego agents are related to vehicle type, which is fixed for the ego agent. Although the $10$ weather attributes are each continuous, we select these vectors from $15$ weather choices during training and so, with regards to the encoding, they each correspond to discrete choices. Similarly, because the camera intrinsics were drawn from the (realistic) discrete Nuscenes~\cite{nuscenes2019} distribution, their encoding is discrete.

The agent tokens have a set order. First is the discrete type (`blueprint'), then the continuous $(x, y, z)$ locations and $(\textrm{roll}, \textrm{yaw})$ rotations. To discretize the locations, we first subtract their minimum possible value. The resulting value is in $[0, 600)$ and we encode it with three tokens $w_k$: $w_0 \in [0, 5]$ represents the hundreds place, $w_1 \in [0, 99]$ the ones, and $w_2 \in [0, 9]$ the decimal. This small sacrifice of precision marginally impacts scene reproduction. Rotation uses the same encoding, albeit it is bounded in $[0, 360)$.

% \james{This is much clearer then before! Though, small point, should $w_0 \in [0,5]$? Is this a standard encoding too?}
% \cinjon{addressed}

%\karsten{If we need to save space later, I think this paragraph here can be shortened with details in appendix. It may be fine to say that the scene graphs are flattened and discretized when necessary and just mentioning the types of attributes with details in Appendix.}

% \subsection{Scoring function}  
\paragraph{Scoring} We require a per-example scoring function $f$ to quantify the intervention delta $\delta = f(\phi, I', L') - f(\phi, I, L)$.
% \ak{might be good to have a notation for intervention $x' \sim I_{MLM}(x)$}
Our goal was to replicate the AP score's intent, which values having few predictions with high intersection over union (IOU) to ground truth targets. Another goal was to evaluate entire scenes and not just target assets. This is important because even though our interventions are local to a node, they may still impact detecting any scene constituent.

We first get the model's predictions and order them by confidence, highest to lowest. We sequentially align each prediction with the highest IOU ground truth. If $\textrm{IOU} > .05$, then we mark this ground truth as claimed. The per prediction score is the product of the prediction's confidence and its IOU. We then take the mean over all predictions to get the model's final score on this example. This penalizes the model for having low confidence or a poor IOU and bolsters it for having high confidence on quality boxes. 

% To get the interventions, we perform the following procedure on $D = 10000$ held out scenes $s_k$. Per $s_k$, pick a single random categorical change, ask the MLM to infer a replacement, and then re-render this new scene $s_{k}^\prime$. Compute delta $\delta = f_{18\textrm{C}4}(s_{k}^\prime) - f_{18\textrm{C}4}(s_k)$ between the score of $f_{\phi}$ on both scenes, where our $\phi$ is a $18\textrm{C}4$ model trained on the base $10000$ subset from Town03. We isolate those that have high absolute score changes ($|\delta| \ge 0.2$) and group them by category, filtering for categories that have at least $20$ entrants.

\paragraph{Summarizing,} we propose finding hard groups for a trained model $\phi$ by taking interventions on scene sequences through the use of an MLM and assessing the results with our own surrogate scoring function $f$. Our MLM infers a new scene close to the original distribution with
% \james{only one at a time? And otherwise from finite set?}
% \cinjon{addressed}
semantic changes such as weather, agent asset type, location, or rotation, and then the scores from $f$ delineates between interventions that were minimal and those that caused a high delta change. The assumption is that high negative delta changes imply that the intervention was deleterious to $\phi$ and high positive changes are the same in reverse. Asserting that a particular scene is hard does not provide any insights into why nor how to fix it; Asserting that a type of intervention is consistently hard narrows greatly where the model's difficulties lie without ever including humans in the process \textit{and} suggests a route to fixing those difficulties. 
% \orl{I like this summary and that's a strong point -- but probably requires some support. Namely, it's not obvious that interventions generalize between scenes. }
%\karsten{I feel this is a very important point here, so I'd finetune this argument a bit. I am wondering whether such a sentence would be nice even in the intro to motivate our approach...} 
After finding this priority list, we address the groups via hard negative mining~\cite{DBLP:journals/corr/abs-1709-02940,DBLP:journals/corr/KumarHC0D17,DBLP:journals/corr/WangSLRWPCW14}, a common technique for improving models by first mining the data for the hardest examples and then emphasizing those examples in the training set by either retraining or fine-tuning. 

% We are working in an AV setting and assume access to a simulator that gives us full information of the scenes. With this, we could try and understand causes by taking naive statistics over a model's results on a held out dataset. We could also train models to yield this insight. However, both face grave computational challenges with respect to the tremendous number of scene permutations in even a single town. 
%Even in the face of this concern, we tried to train a model to gauge the score from a scene and found its reliability lacking. See the Appendix for a summary.





%%%
%%% Cinjon previous ...
%%%

% Figure~\ref{fig:exp7-validate} compares the performance of trained models on held-out data sampled from the training distribution and held-out data with increased occurrence of a challenging instance type, Diamondbacks, which are a brand of bikes. We are motivated to find similarly challenging modes with limited human involvement, especially modes that are not so easily hypothesized as the Diamondbacks.

% One approach to doing this would be to iterate through the training set and gather examples for which the model gives poor results. One concern with this is what metric to use to decide whether an example is challenging; AP and other common detection metrics operate over a full dataset and not a single example. A more pressing concern is that this iteration only tells us whether an example is problematic without providing any insight into the underlying cause. The actual cause is opaque because the number of interventions in a scene scales combinatorially with the number of possible interactions among constituents like agents, time of day, cloudiness, rain, etc. Understanding those causes helps us in both finding more data that would patch the deficiency but also in grokking whether we have sufficiently addressed the issue. 

% \subsection{Causal interventions on simulated scenes}

% We take inspiration from causal inference where interventions allow us to assess the causal links between the scene and the model's score. We propose to do that here by first assuming access to an AV simulator that gives full information of the scenes such that we can re-sample as desired by, for example, changing the rotation or location of a specific car. We then take interventions on those scenes and assess which kinds cause deleterious changes  $\delta$ to the model's score. After applying a threshold to the $\delta$ and grouping the resulting intervention by type, we arrive at an ordered list of challenging modes at the semantic level of specific rotations, car types, or weather patterns.

% An immediate issue is that if we take a completely random intervention, then when we assess the model's performance, we do not know if we are producing data on the distribution or not. This is a confounder for drawing conclusions about the difficulty of the example with respect to its actual utility in improving our model. In other words, we would like for the model to be able to detect flying cars, but given a computational budget, that out-of-distribution mode is much lower priority than detecting motorbikes in the dark, and so we should favor finding the latter over the former. \orl{i'd consider removing the next comment to get to the point faster.} This is especially true for a limited model capacity because learning to detect flying cars and other unrealistic low-priority scenarios will take capacity away from pressing needs; it is also true in practice because detection labeling is expensive and our budget is never infinite.

% Formally, if $p(x)$ is the (scene) generation process, $y$ is our surrogate score, and $z$ is a confounder that affects both $x$ and $y$ 
% %(e.g. weather, assets, their positioning, and combinations thereof)
% , then we need to draw an $x^\prime$ that is independent of $z$. Sampling from $p(x)$ is challenging because retrieving the same scene again with just one change is difficult. Instead, we train a denoising autoencoder (DAE) to sample faithfully from $p(x)$~\cite{DBLP:journals/corr/abs-1305-6663,DBLP:journals/corr/abs-1905-12790,10.1145/1390156.1390294}. For our needs, this is best satisfied by using a masked language model (MLM) as our DAE~\cite{DBLP:journals/corr/abs-2009-10195,DBLP:journals/corr/abs-1902-04094} where the MLM was trained on flattened sequences representing the scene graphs.\orl{are masks taken also of a single node? or arbitrary number of nodes? maybe let's explain to the reader how this training looks like, loss functions and all? Like Karsten said, if this goes to a vision paper, even the idea of training a scene graph as language model is not going to be intuitive.}

% Figure~\ref{fig:scenegraphconversion} shows how we convert the scene graph $G$ to a flat sequence $S$ where the discrete tokens are representations of the weather, agent asset types, rotations, and locations. \orl{details to follow. } We use these sequences to train the MLM. At inference, we input new sequences to this model and re-sample a single masked token to create new scenes. Because the model was trained to a low perplexity on data drawn from the distribution, it can faithfully sample from the original distribution $p(x)$. Of course, our model is not the exact distribution and so errors will accumulate when running for many interventions in sequence. Therefore, we run for just one categorical step, which is equivalent to a single node change in the scene graph.
% % Motivated by contrastive divergence\cite{10.1162/089976602760128018}, we run for just one categorical step, which is akin to a single intervention.

% \paragraph{Scene-sequence encoding} Encoding the language requires us to translate a scene graph $G$ with continuous node attributes into a discrete sequence $S$. The first $10$ tokens correspond to the weather attributes\footnote{Cloudiness, Precipitation, Sun Altitude Angle, etc}, the next $5$ tokens are camera intrinsics, and the following $15$ tokens represent the ego agent. After these $30$, we have a variable number of agents, each represented sequentially by $17$ tokens. The two extra tokens for the agents are related to the ego agent's vehicle type being fixed.

% Although the ten weather attributes are each continuous, we select from $15$ weather choices during training and so, wrt the encoding, they each correspond to discrete choices. Similarly, because the camera intrinsics were drawn from the (realistic) Nuscenes~\cite{nuscenes2019} distribution, they also have a discrete set of choices and so their encoding is also discrete.

% The agent tokens have a set order. First is the discrete type (`blueprint'), then comes the continuous $(x, y, z)$ locations and $(roll, yaw)$ rotations. In order to discretize the locations, we first subtract their minimum possible value to bound them below by $0$. The resulting range is in $[0, 600)$ and so we encode then with three tokens $w_k$ where $w_0 \in [0, 6]$ representing the hundreds place, $w_1 \in [0, 99]$ representing the ones, and $w_2 \in [0, 9]$ representing the first decimal. This small sacrifice of precision does not appear to hurt us in reproducing scenes. Rotation is similar and uses the same encoding, albeit it is bounded in $[0, 360)$.
% %\karsten{If we need to save space later, I think this paragraph here can be shortened with details in appendix. It may be fine to say that the scene graphs are flattened and discretized when necessary and just mentioning the types of attributes with details in Appendix.}

% \subsection{Scoring function} We have need for a per-example surrogate scoring function $f_{\phi}$ in order to quantify the delta change in an intervention. Our goal was to replicate the intent of the AP score, which values having few predictions, each with high intersection over union (IOU) to a ground truth target. We first get the model's predictions and order them by confidence, highest to lowest. We sequentially align each prediction with the highest IOU ground truth. If $\textrm{IOU} > .05$, then we mark this ground truth as claimed. The per prediction score is the product of the prediction's confidence and its IOU. We then take the mean over all predictions to get the model's final score on this example. This penalizes the model for having low confidence or a poor IOU and bolsters it for having high confidence on quality boxes. \orl{there's a point here that might worth discussing. Even though our intervention can be local, like rotating a car, it may still damage detection of other assets. I'd start with this maybe, to motivate why our scoring function is global. Of course, there's also global change like weather.  }

% To get the interventions, we perform the following procedure on $D = 10000$ held out scenes $s_k$. Per $s_k$, pick a single random categorical change, ask the MLM to infer a replacement, and then re-render this new scene $s_{k}^\prime$. Compute delta $\delta = f_{18\textrm{C}4}(s_{k}^\prime) - f_{18\textrm{C}4}(s_k)$ between the score of $f_{\phi}$ on both scenes, where our $\phi$ is a $18\textrm{C}4$ model trained on the base $10000$ subset from Town03. We isolate those that have high absolute score changes ($|\delta| \ge 0.2$) and group them by category, filtering for categories that have at least $20$ entrants.


% \textbf{Summarizing}, we propose finding hard modes for a trained model $\phi$ by taking interventions on scene sequences through the use of an MLM and assessing the results with our own surrogate scoring function $f_{\phi}$. Our MLM can infer a new scene close to the original distribution with any number of semantic changes such as weather, agent asset type, location, or rotation, and then the scores from $f_{\phi}$ can delineate between interventions that were minimal and those that caused a high delta change. The assumption is that high negative delta changes imply that the intervention was deleterious to the model's capability and high positive changes are the same in reverse. Asserting that a scene is hard does not provide any insights into why nor how to fix it; Asserting that a type of intervention is consistently hard narrows greatly where the model's difficulties lie without ever including humans in the process and suggests a route to fixing those difficulties. 
% % \orl{I like this summary and that's a strong point -- but probably requires some support. Namely, it's not obvious that interventions generalize between scenes. }
% %\karsten{I feel this is a very important point here, so I'd finetune this argument a bit. I am wondering whether such a sentence would be nice even in the intro to motivate our approach...} 
% After finding this priority list, we can address the modes via hard negative mining~\cite{DBLP:journals/corr/abs-1709-02940,DBLP:journals/corr/KumarHC0D17,DBLP:journals/corr/WangSLRWPCW14}, a common technique for improving models by first mining the data for the hardest examples and then emphasizing those examples in the training set by either retraining or fine-tuning. 

% % We are working in an AV setting and assume access to a simulator that gives us full information of the scenes. With this, we could try and understand causes by taking naive statistics over a model's results on a held out dataset. We could also train models to yield this insight. However, both face grave computational challenges with respect to the tremendous number of scene permutations in even a single town. 
% %Even in the face of this concern, we tried to train a model to gauge the score from a scene and found its reliability lacking. See the Appendix for a summary.







==> core/prior_versions/5_experiments.tex <==
\section{Experiments}
\label{sec:experiments}

This section introduces a litany of experiments showing the virtue of our proposed method, as well as support for random interventions being less efficient than our method.

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.47\textwidth]{imgs/exp7/18_C4_1x.both.justbig..h3.750.png}
    \caption{Test results with config $18\textrm{C}4$ when training on disjoint IID subsets. Results are consistent, suggesting that the harder groups - bikes, rotations, and cybertruck - are ubiquitously hard.}
    \label{fig:exp7-18c4}
\end{figure}

\subsection{Datasets}
To create the datasets, we first select the CARLA preset map, either Town03 or Town05. Then we randomly choose from among the pre-defined weather patterns. We randomly select the camera calibration and the number $V$ of vehicle assets according to the distributions in Nuscenes. We place those $V$ vehicles, the ego agent, and $P = 20$ pedestrian assets, at random town waypoints suitable for the asset type. Finally, we attach the calibrated camera to the ego agent and set every agent to autopilot.

We wait for $50$ timesteps after spawning so the scene stabilizes. We then record for $150$ steps and save every $15$th frame. We need the 2D ground truth boxes for each asset, but found the suggested approach\footnote{See client\_bounding\_boxes.py in the CARLA repository, commit hash 4c8f4d5f191246802644a62453327f32972bd536.} lacking because it frequently has trouble with occlusions and other challenging scenarios. See the Appendix for heuristics we developed to help filter the ground truth boxes.

%%%%
%%% Cinjon - maybe should add this back in?
%%%%

% \paragraph{Is there a challenging mode?}

% Figure~\ref{fig:exp7-validate} shows the AP scores of a trained detection model on held out datasets of Diamondback bikes and IID data. The results are poor on the former and strong on the latter. As mentioned in Section~\ref{sec:method}, we had a prior that this would be so because the training dataset distribution of bikes in Nuscenes is low. That there is an issue due to data imbalance is not uncommon in machine learning systems, and here we establish that about our own. We will now search for these modes systematically with our proposed method.

%%%%

\subsection{Interventions}

\begin{table}[!t]
\centering
\begin{tabular}{c|c|c}
Intervention & Percent $> 0.2$ & Total \\
\hline
\multicolumn{3}{c}{Tier 1: Likely Challenging Groups} \\
\hline
DiamondbackBike & 24.4 & 123 \\
Cloudy Dark & 19.4 & 36 \\
GazelleBike & 18.9 & 122 \\
Cloudy Dark Puddles & 17.2 & 29 \\
CrossBike & 16.5 & 121 \\
Rotation - 178.6 & 15 & 20 \\
Rotation - 121.3 & 13.0 & 23 \\
\hline
\multicolumn{3}{c}{Tier 2: Borderline Groups} \\
\hline
KawasakiBike & 6.5 & 92 \\
Cybertruck & 6.4 & 94 \\
Carla Cola & 6.0 & 198 \\
Sunny Puddles & 5.4 & 56 \\
\hline
\multicolumn{3}{c}{Tier 3: Easy Groups} \\
\hline
Citroen C3 & 1.6 & 188 \\
Mercedes CCC & 1.0 & 206 \\
\end{tabular}
% \vspace{-1mm}
\caption{Illustrative table of selected interventions, ordered by the percent of times that they were involved in a high magnitude $\delta$ event. The 2nd column shows that percent and the 3rd column the total number of observations. Section~\ref{sec:experiments-analysis} suggests that between 6.0 (Carla Cola) and 6.4 (Cybertruck) is where our cutoff should lie.}
\label{table:intervention}
\vspace{-4mm}
\end{table}

Table~\ref{table:intervention} shows selected ordered results from the intervention procedure described in Section~\ref{sec:method}. We performed the procedure on $N = 10000$ held out scenes $G_k$ where our $\phi$ is an $18\textrm{C}$ model trained on the base $10000$ subset from Town03 and $\tau = 0.2$. We additionally filter the categories to have at least $20$ entrants.

On the left side we see the intervention taken, for example changing a single agent type to a Cybertruck or changing the weather such that it is now sunny with reflective puddles. 
%For the former, this would be changing one `word' representing the NPC's type in a scene sentence to the word `26'; our system would know to then render that vehicle as a Cybertruck instead of the previously specified vehicle while maintaining the same rotation and location. For the latter weather, this would be masking out all words representing the weather and letting the MLM sample such that cloudiness, precipitation, precipitation deposits, wind intensity, and sun altitude angle are now encoded with the words corresponding to a sunny environment with puddles. 
The second column shows the probability that the intervention produced a $\delta \ge 0.2$. We include both when the change was \textit{to} that target and the delta was negative as well as when it was \textit{from} that target and the delta was positive. The last column in the table reports how many times in total this intervention occurred in the $10000$ scenes.

Summarizing the table, we find that a handful of asset switches appear to be deleterious groups for the model according to this metric. In particular, `small bikes' have an outsized effect, as does cloudy weather and the rotations where a car is coming at the ego agent or turning to the left. Just after the last bike are two large vehicles, the Cybertruck and the Cola Car. The specificity of the listed weathers and rotations are due to our discretization gifting us an exact value that we translate in the table for semantic understanding. Practically speaking, there is a range of rotation and weather values around the group that would all suffice.

Finally, we do not include any location results in this table because the MLM would frequently re-position the asset somewhere out of the camera's purview. This says more about the asset than it does about the location, and it is also rife with confounders based on what was behind that asset. 
% \james{I don't follow this last sentence. If I understand right, this suggests that the location interventions should just be more constrained so they can't remove the object from view?}
% \cinjon{Agree. recognized below}
We could have localized the location interventions more by zeroing out MLM options, but leave that for future work. 
% \orl{so we first say that the early in the research, we thought Diamondback bikes are going to be a hard mode due to their poor representation in the data. Then we propose intervensions as a way to find other important modes. Do we show that these other modes can't be as easily found by looking at their representation in the data?}
% \cinjon{i tried to address this by saying in the Diamondback section that we didnt have insight into others except bikes}


\subsection{Analysis}
\label{sec:experiments-analysis}

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.47\textwidth]{imgs/exp1and2.0.combined.h6.png}
    \caption{Charts showing independently increasing the model capacity (left) and increasing the data size (right). We see that no model distinguished themselves and that we quickly taper in how effectively the model utilizes the data. We consider the dip in the capacity chart to be an artifact of the training procedure and using the same settings for all of the models.}
    \label{fig:exp1and2-18-10k}
\end{figure}


After obtaining candidate groups from the designed interventions, we investigate the effect of modifying the data sampling procedure to increase the prevalence of these groups by building and evaluating datasets sampled from the MLM training set. For asset groups, for each datum, we uniformly sample $n_{\textrm{v}} \in [3, 6]$ as the number of vehicles selected from the scene. We then randomly choose vehicles $v_0, v_1, \ldots, v_{n_{\textrm{v}}}$ in that scene, including vehicles that may actually not be in the camera's purview, and change them to be the target mode. So as to not accidentally introduce a bias through the random process, we select the same vehicles $v_k$ for all group datasets.
% \karsten{This may be a dumb question, but why exactly is that? Don't different scenes have different cars? Couldn't we just each time change some cars to mode? Not sure I understand this correctly}. 
% \cinjon{Adjusted to make the meaning more clear. Each time we are changing the same cars. I think the confusion was in that we change it per scene.} 
% \orl{i feel that last sentence is still unclear. }
% \cinjon{how about now?}
For rotation groups, we choose those same vehicles but rotate them to be the target rotation instead of switching their asset. For weather groups, we change those scenes to have the target weather instead.

\begin{figure*}[!t]
    \centering
    \includegraphics[width=\textwidth]{imgs/exp3&6/exp3and6.18C4.rowcol.s0-e20000.h7.png}
    \caption{Results of training $18\textrm{C}4$ on the base IID $10000$ training set plus additional group data. The five groups in the top left (Cybertruck, Cola Car, Diamondback, Gazelle, and Crossbike) are added equally. Observe that, for all charts, adding any one group improves all of the other evaluation scores, and at no point do we lose efficacy on the IID data as a whole. Figure~\ref{fig:exp3-configs-0-1k} (Appendix) zooms in on the initial jump.}
    \label{fig:exp3-configs-0-20k}%
\end{figure*}

\begin{figure}[!h]
    \centering
    \includegraphics[width=0.47\textwidth]{imgs/exp.2-3.bothconfigs.samedataiid.zoomed.start10k.h6.png}
    \setlength{\belowcaptionskip}{-10pt}
    \caption{How much IID data is required to match a small amount of extra hard group data. The top left shows $20000$ more IID data is required to reach par on IID with $250$ group data. The bottom left shows that we never reach the same level on Diamondbacks with IID data as with adding Cybertrucks, let alone actual bikes.}
    \label{fig:exp23-iidmodes}%
\end{figure}

\paragraph{Does our method correlate with AP score?} Figure~\ref{fig:exp7-18c4} shows evaluation results on these groups when training $18\textrm{C}4$ on four disjoint $10000$ sized subsets of the data. The models perform best on the IID data from Town03 and just a little bit worse on the same from Town05. Further, they do exceptionally well on those two datasets, validating that they were trained sufficiently.

The group results are mostly in line with our expectations from the interventions - the models do well on Citroen and Mercedes, poorly on the rotations, and terribly on the bikes. There is a large jump from the reasonable results on ColaCar and SunnyPuddles to the mediocre results on Cybertruck, which is directionally correct per Table~\ref{table:intervention}. However, the strong results on CloudyDark are surprising.

\textbf{Summarizing}, if the threshold for choosing a group is between $5.5\%$ and $6.5\%$ and we focus on interventions affecting vehicles directly (rotation and type), then our method correlates well with empirical results. This does not mean that we have found the exact causes of the model's issues, but that we have narrowed them greatly. The model's regression when changing a car to a bike may be because it performs poorly on bikes. It may also be because the car was occluding another vehicle or that it itself was not occluded. This is especially true in light of the weather results suggesting that weather is not a conclusive factor. Finding the exact cause is a difficult problem, even in simple settings~\cite{arjovsky2020invariant}. We restrict our scope to this level of understanding and leave improvements for future work.

\paragraph{Can we address these issues by increasing capacity?} Recent papers~\cite{zhai2021scaling,DBLP:journals/corr/abs-2102-06701} suggest that scaling our models will improve results. An affirmative answer would mean we would not need to collect more data. While it is possible that we did not scale enough or use the right architectures, the left side of Figure~\ref{fig:exp1and2-18-10k} suggests a negative answer.
% \orl{let's give more details about the models and their capacity. Maybe parameter count?} 
% \cinjon{appendix from earlier on}
We see that no model was distinguished with respect to their final values when using $10000$ IID examples.

\paragraph{What if we increased IID data?} While we would have to collect data, this would be easier to attain than group specific data. The right side of Figure~\ref{fig:exp1and2-18-10k} suggests this too will not be sufficient. We see an initial jump from $1000$ to $10000$ IID data points, but efficacy slows precipitously across town and group data. We have no reason to think this will suddenly change, and Figure~\ref{fig:exp.3&4-18_C4} (Appendix) affirms that by suggesting that the percentage of representation of the group is what matters, rather than absolute count.

\paragraph{What if we increased data and capacity simultaneously?} Results remain negative, as seen in Figures~\ref{fig:exp1and2-34-85k} and \ref{fig:bothoverlay} (Appendix). The left graphic in Figure~\ref{fig:exp1and2-34-85k} evaluates all of the models on $85000$ examples and the right one hones in on the $34\textrm{C}4$ model, showing its results across a range of IID data counts. Three aspects stand out. The first was that all of the models have similar evaluation scores. The second is that they all struggle on the harder groups. And the third, seen more clearly in Figure~\ref{fig:bothoverlay}, is that more data yields a small accretive effect. This suggests that, all else equal, adding data may be better than adding model capacity. 
% \karsten{I am wondering whether this could go into appendix. It's exactly what one would expect given the previous two paragraphs and doesn't add much new insights (Figs. 4 and 5 look extremely similar). Some of the discussion, for example that adding data seems better, could be added to the above ones.}
% \orl{i tend to agree. We could also keep this and put the previous in the appendix if this one is more impressive. }
% \cinjon{discussed offline and how we shoudl keep it}

\paragraph{Using group data} We expect that when we add data from the groups to the training set that we will address the issues. The top left plot in Figure~\ref{fig:exp3-configs-0-20k} confirms that to be true. We add an even amount of each group to the base $10000$ IID subset and see that every group improves without impacting the Town03 and Town05 results.

The other plots in Figure~\ref{fig:exp3-configs-0-20k} show what happens when we add in training data from any one group $M$. This predictably improves the model's results on $M$'s validation set. It surprisingly also improves results on \textit{all} of the other groups $M^\prime$ and the Town data. The improvement to $M^\prime$ is smaller than that to $M$, but it is notable. The gains for a specific group are more pronounced for like groups - adding data from a biker group (Diamondback, Omafiets, Crossbike) improves the other biker groups a lot more than adding data from the heavy car groups (Cybertruck, Colacar), and similarly for the heavies. Adding rotation groups helps ubiquitously albeit not as much as adding a bike group does for the other bikes. The least effective fix is adding the CloudyDark weather mode. Figure~\ref{fig:exp.3&4-18_C4} shows that this trend persists for a base of $85000$ IID data as well. 

\paragraph{Comparison with random interventions}

As we alluded to in Section~\ref{sec:method}, taking random interventions is problematic because whether the group is reasonable for the distribution will be a confounder. We wish to prioritize the found groups to be those that are more likely seen in the wild. We show here that this is true by taking the $10000$ source scenes used for the MLM interventions and applying random manipulations of the same type. For example, if we changed agent $a_j$'s vehicle type in $G_k \rightarrow G^{\textrm{MLM}}_k$, then we change $a_j$ to a random vehicle type in $G_k \rightarrow G^{\textrm{Random}}_k$. 

% We took the $10000$ source scenes used for the MLM interventions and applied random manipulations of the same type. For example, if we changed agent $a_j$'s vehicle type in $G_k \rightarrow G^{\textrm{MLM}}_k$, then we changed $a_j$ to a random vehicle type in $G_k \rightarrow G^{\textrm{Random}}_k$. In Table~\ref{table:random} and Figure~\ref{fig:intervention_kde} (Appendix), we show results for asset, weather, and rotation changes. Assets are analyzed similarly to the MLM interventions because they are symbolic. For rotation and weather, we show density plots to demonstrate the differences because they are continuous for random interventions.

\begin{table}[!t]
\centering
\begin{tabular}{c|cc|c}
Intervention & MLM & Random & Random Total \\
% \hline
% \multicolumn{3}{c}{Tier 1} \\
\hline
CrossBike & 16.5 & 19.0 & 126 \\
GazelleBike & 18.9 & 18.7 & 171 \\
DiamondbackBike & 24.4 & 15.8 & 152 \\
% \hline
% \multicolumn{3}{c}{Tier 2} \\
\hline
Carla Cola & 6.0 & 8.1 & 210 \\
Cybertruck & 6.4 & 6.8 & 176 \\
KawasakiBike & 6.5 & 6.6 & 121 \\
% \hline
% \multicolumn{3}{c}{Tier 3} \\
\hline
Citroen C3 & 1.6 & 3.5 & 197 \\
Mercedes CCC & 1.0 & 3.8 & 183 \\
\end{tabular}
% \setlength{\belowcaptionskip}{-10pt}
\caption{Results for MLM and Random asset intervention strategies, ordered by the percent of times that they were involved in a high magnitude $\delta$ \textit{random} event. While the top three types are the same, Random flubs the dividing line by placing a) Cybertruck above Kawasaki Bike and b) Carla Cola well ahead of both. Additionally, its failure rate for the easy cars is much higher and, in general, posits 3\% more failures than MLM. All told, its results would create a lot more work for human verification and testing and vastly reduce the degree of automation that we could employ to find the hard modes.}
\label{table:random}
\vspace{-4mm}
\end{table}

Table~\ref{table:random} shows results for random and MLM interventions over the same assets specified in Table~\ref{table:intervention}. One immediate observation is that the assets are ordered incorrectly with CarlaCola higher than both Cybertruck and Kawasaki Bike. Another observation is that Random has a higher percent of high threshold events. This holds in general, with $13.2\%$ of random interventions impacting the model versus $10.2\%$ of MLM interventions. We hypothesize this is because random re-sampling of elements of the scene graphs corresponds to sampling from a data distribution that does not faithfully represent the original training distribution. While this $3\%$ may appear to be a small difference, it is very large with respect to how much extra work would be required by people combing through and seeing if the data is actually plausible and should be accounted for in retraining.

Figure~\ref{fig:intervention_kde} (Appendix) shows density plots for rotation and cloudiness interventions, conditioned on the intervention being deleterious. We use density plots to demonstrate the differences between Random and MLM because these interventions are continuous for Random. For rotation, we see that there is a mostly steady plateau for Random while MLM shows a clear single group aligned with the bi-modal humps in Original. For weather, we see that Original and MLM are almost overlapping and, while Random is similarly bi-modal, its shape is less pronounced and more even as expected. These both further reinforce our claim that the advantage of MLM is that it gears us towards higher priority groups to fix that are in line with the actual data distribution. 

\paragraph{Qualitatively, why do these groups exist?} With groups in hand, it is now easy to ascertain why our models were failing. For the bikes, it is because they are underrepresented in Nuscenes. For Rotation121, the model infrequently trains on turning cars due to the town layout. For Rotation178, the model infrequently trains on cars facing it due to the traffic policy and the quantity of cars. The Cybertruck is challenging because it is very large and causes occlusion issues in labeling. The ColaCar also has this issue, just not as severely as the Cybertruck. These issues can only be hypothesized without the groups in hand.


% 1. Why are thevikes and the rotations and the large truck bad? The rotation is because it's underrepresented in the Dara ... The bikes are because of label error... The large tricks is because of what happens as you get closer to the truck. but this is normal! all real world data looks this messy … it comes from some distribution and is labeled w some distribution. this is also why random is a bed way to do this because it ignores the real issue that is priority of the what data to go retrieve 

% get histogram if cars in both random and in beer and in original 
% do same for rotations


% \pagebreak





==> core/prior_versions/unused_4_method_ver2.tex <==
\section{Method (V2)}
\label{sec:method}

\james{Reading through this section more carefully, I feel that there is quite a lot of repetition between the second and third paragraphs and the last two. I would suggest that we use the second paragraph to describe the overall scheme. Then describe the scoring function (basically copy-and-paste the "Scoring function" paragraph), and then describe the causal interventions with the MLM by combining the current third and}

We aim to improve object detection models by utilizing the advantages of AV simulators over collecting real world data, namely that they quickly synthesize scenes in parallel and that we have fine control over the synthesis. A naive approach is to generate lots of scenes, test detection on those scenes, and set aside the hard ones for retraining. \orl{To go beyond naive approahces, I think we can also say that even adversarial attacks would find sporadic, unexplained failures.} This fails for a number of reasons, but the most important are a) we are much more interested in plausible scenes than implausible ones, and b) we still have the combinatorial challenge of understanding what in the scenes was the problem. Only if we know why the error is happening can we understand if it is fixed after we retrain.

We propose an efficient procedure that tackles both of these concerns. We find hard groups of data for a trained model $\phi$ by taking interventions on scene sequences through the use of a pre-trained MLM and assessing the results with our surrogate scoring function $f$. For each scene drawn from the original training distribution, the MLM infers a new scene close to the original distribution by making a singular semantic change over weather, vehicle asset type, rotation, or location. Because the MLM was trained to a low perplexity on data drawn from the distribution, it faithfully samples from the original distribution $p_{\textrm{R}}(x)$ \james{this feels like a technical claim that we can't guarantee. Suggestion: "it samples scenes that are likely under the original distribution $p_{\textrm{R}}(x)$"}. Because it is not the exact distribution and errors will accumulate when applying many interventions sequentially, we intervene for just one step, equivalent to a single node change in the scene graph. Observe that we could act directly on the scene graph and model the conditional distributions of a single node change, then select changes via Gibbs sampling, and define interventions as sampling from these conditional distributions. We choose to instead use discretization~\citep{oord2016wavenet,DBLP:journals/corr/EngelRRDESN17,razavi2019generating} and masked language models~\citep{dosovitskiy2021image,khan2021transformers} because of their increasing success in modeling the distribution, demonstrated so clearly in language.

We use $f$ to delineate between interventions that were minimal and those that caused a high delta change \james{we don't define delta until a few paragraphs later. Maybe replace "delta change" with "score change" here?}, with the assumption being that high negative (positive) delta changes imply that the intervention (reverse intervention) was detrimental to $\phi$. Asserting that a \textit{scene} is hard does not provide any insights into why nor how to fix it, but asserting that a type of \textit{intervention} is consistently hard narrows greatly where the model's difficulties lay and suggests a route to fixing those difficulties. Importantly, our approach achieves this without relying on humans in the loop. After finding this priority list, we address the groups via hard negative mining~\citep{DBLP:journals/corr/abs-1709-02940,DBLP:journals/corr/KumarHC0D17,DBLP:journals/corr/WangSLRWPCW14}, a common technique for improving models by first mining the data for the hardest examples and then emphasizing those examples in the training set by either retraining or fine-tuning. 
We now explain in detail each of the components of our method.

\vspace{-12pt}

\paragraph{Scoring function} Our goal for the per-example scoring function $f$ is to replicate the AP score's intent, which values having few predictions with high intersection over union (IOU) to ground truth targets. Another goal was to evaluate entire scenes and not just target assets. This is important because even though our interventions are local to a node, they may still impact detecting any scene constituent. We choose not to use mAP because it is only defined over a full dataset and thus it would be confusing in this context \james{suggestion: "it would be confusing in this context" $\rightarrow$ "is not suitable for identifying challenging examples"}. We first get the model's predictions and order them by confidence, highest to lowest. We sequentially align each prediction with the highest IOU ground truth. If $\textrm{IOU} > .05$ \james{minor: is this value standard/otherwise justified}, then we mark this ground truth as claimed. The per prediction score is the product of the prediction's confidence and its IOU. We then take the mean over all predictions to get the model's final score on this example. This penalizes the model for having low confidence or a poor IOU and bolsters it for having high confidence on quality boxes. 

\vspace{-12pt}

\paragraph{Causal interventions on simulated scenes}
We draw from causal inference where interventions allow us to assess the causal links between the scene and the model's score. We change an aspect of a scene sequence $S_i$, such as a rotation or location of a specific vehicle, render this new scene $S_{i}^\prime$ as $I^\prime$, and then compute the $\delta = f(\phi, I^\prime, L^\prime) - f(\phi, I, L)$. If $\delta$ is sufficiently negative (positive), then the target (original) attribute in the intervention is potentially problematic for $\phi$. We decide sufficiency by whether $|\delta| \ge \tau$, the aforementioned threshold parameter. After performing this procedure $N$ times, filtering by sufficiency, and then grouping by the intervention type, we arrive at a prioritized list of challenging groups defined by either rotation, vehicle type, or weather pattern.
% \orl{that last part of grouping is not clear. it sounds like we're discovering intervention groups but really we're prioritizing among a pre-defined set of intervention groups. Maybe fist define these groups as types of interventions in the notation section, and then here we can discuss ranking them more formally?}

\vspace{-12pt}

\paragraph{Generating interventions using an MLM}
Intervening randomly produces unlikely scenes under the true data distribution. Even if such an intervention would identity a weakness in the detector, its utility in improving our model is unclear because such a weakness may be very far from a realistic setting. We should favor finding groups that have higher probability under the distribution. This is especially true for a limited model capacity because learning to detect flying cars and other unrealistic low-priority scenarios will take capacity away from pressing needs. Formally, with $p_{\textrm{R}}(x)$ as the generation process, $y$ our surrogate score, and $z$ a confounder that affects both $x$ and $y$, we need to draw a counterfactual $x^\prime$ that is independent of $z$ with which we can causally probe the model's weaknesses. Sampling from $p_{\textrm{R}}(x)$ is challenging because retrieving the same scene again with just one change is difficult. Instead, we train a denoising autoencoder (DAE) to sample from $p_{\textrm{R}}(x)$~\citep{DBLP:journals/corr/abs-1305-6663,DBLP:journals/corr/abs-1905-12790,10.1145/1390156.1390294}. This approach of sampling counterfactuals from the data distribution is satisfied by using a MLM as our DAE~\citep{DBLP:journals/corr/abs-2009-10195,DBLP:journals/corr/abs-1902-04094}, where the MLM operates on sequential discretized scene graphs.
% \orl{please simplify this. maybe also give a concrete example.}
% \orl{now i'm missing an explanation on how MLM work. Let's say whats the input and output so that we position them as the perfect candidate with the only caveat being they're not made for graph but for sequences. This should set the ground for explaining the graph flattening.}


\begin{figure}[!h]
    \centering
    % \captionsetup{type=figure}
    \includegraphics[width=0.9\textwidth]{imgs/explainpic-group.png}
    \caption{\textbf{A complete diagram of our approach}: We intervene on the scene by performing transformations like the pictured yellow truck becoming a white car and then evaluating the delta change in the object detection model's efficacy. The interventions are guided by a trained MLM. Repeat 10000 times and group the scores to attain an ordered list of challenging groups drawn from vehicle type, weather, and rotation.
    }
    \label{fig:scenegraphconversion}
\end{figure}




==> core/unused/5_experiments_mnist.tex <==
% \section{MNIST}

% We use MNIST to test how our learned model would fare against an oracle as well as what are good strategies for reintroducing the mined examples back into the training process.

% \paragraph{Dataset} We built a data generator where each generated example contains two MNIST digits somewhere on a $100 \times 100$ black background. The label was a $0$ if the digit on the left was less than the digit on the right and a $1$ if the digit on the left was greater than the digit on the right. 

% This generator creates examples by drawing samples from independent distributions on assets (MNIST training data), rotations, and placements, with each using the same starting seed of $0$. There are three distributions: training, $\textrm{validation}_1$, and $\textrm{validation}_2$. We do this to simulate how a perception module trains on only a portion of the real world data and further, how within those portions it sees a skewed set of examples. Accordingly, the $\textrm{validation}_1$ distribution assesses the model's performance when the skew is relaxed and the $\textrm{validation}_2$ distribution grades the model when it sees even more of the universe of data. The distribution specifics are as follows:

% \begin{itemize}
%     \item \textbf{Assets} The training distribution for assets has weight on $1500$ different assets for each of the digit classes. We first randomly determine which digits. We then choose the weights for the chosen digits randomly from the range $[0.75, 1.0]$. The $\textrm{validation}_1$ has equal weight on all of the chosen digits. The $\textrm{validation}_2$ distribution has equal weight on all assets, not just the $1500$ chosen for training.
%     \item \textbf{Rotations} The training distribution for rotations puts a random weight on all rotations in $[-22, 22]$, chosen from the range $[0.1, 2.0]$. The $\textrm{validation}_1$ distribution puts equal weight on all rotations in the same range, while the $\textrm{validation}_2$ distribution includes all rotations in the range $[-30, 30]$, with equal weight on all. 
%     \item \textbf{Placement} The training distribution for placement puts a random weight chosen from the range $[0.1, 2.0]$ on each of the 12 entries in np.linspace(0, 100-28=72, 12). This is used to select each of $x$ and $y$ for every digit. The $\textrm{validation}_1$ distribution puts equal weight on the same range, while the $\textrm{validation}_2$ distribution has equal weight on all 24 entries in np.linspace(0, 72, 24).
% \end{itemize} 

% On each epoch, we draw $60,000$ times from each distribution to train the model. We do the same for each validation at the end of the epoch. The drawn samples satisfy the following constraints:

% \begin{itemize}
%     \item The two digits are from different classes.
%     \item The entire $28 \times 28$ digit is visible.
%     \item At least one of the $x$ and $y$ coordinates have a gap between them. This gap is $10$ for the training and $\textrm{validation}_1$ distributions, and $5$ for the $\textrm{validation}_2$ distribution.
% \end{itemize}


% \paragraph{Model} We then trained a perception model P30 as a neural network via supervised learning with this setup. The model is fed the examples in batches of 64, trains for 20 epochs, and we observe that it attains $98.4\%$, $97.4\%$, and $94.5\%$ accuracies on training, $\textrm{validation}_1$, and $\textrm{validation}_2$. \cinjon{TODO: put in graph below}, with there always being (expected) gaps between both training and $\textrm{validation}_1$, as well as $\textrm{validation}_1$ and $\textrm{validation}_2$.

% \subsection{Miner}

% We freeze P30 and use it as a target for another model, the `miner'. The miner's goal is to find hard examples on which P30 fails. We condition the miner on examples from the training distribution and ask it to take either one or two actions on drawn samples in order to effect the highest impact on the perception module. This is a toy environment simulating drawing examples from real-world perception datasets and then making semantic changes to some aspect of them in order to find where the perception module is weakest. We explore three types of Miners: 1) RLMiner, a learned model that uses vanilla policy gradient loss to learn what to change, 2) OptimalMiner, an oracle that checks every possible change to see what has the biggest effect, and 3) RandomMiner, who takes random (valid) actions.

% The input to both are batches of scene graphs sampled from the training distribution. These contain the tuple of categorical inputs (MNIST class, MNIST index, x position, y position, rotation) for each of the left and right assets. 

% Conditioned on this batch, the OptimalMiner searches through every possible valid change and reports the one that returns the maximal impact to the perception module. It is subject to the constraint that it cannot change an asset to another class, cannot break the constraints we placed on $\textrm{validation}_2$, and cannot move the left digit beyond one before the right digit's $x$ coordinate (rewrite). One consequence of this is that the label will remain unchanged. Note that this may not actually succeed in flipping P30's prediction.

% The RLMiner has a similar object and constraints, but computes its choice of what to change by using a policy (neural) network. For each tuple in the scene graph, it chooses an independent embedding for each of the five entries in the tuple. It concatenates these five together and inputs that to a two layer MLP with hidden size 64 and ReLU nonlinearity. It then concatenates the representations of the two tuples and runs that through another two layer MLP (same hiddens ize and nonlinearity) before running this output through a final linear layer. The policy has dimension 2 + 3 + max([num rotations out, num translations out, num assets out]). This is because we do ancestral sampling where the first two outputs represent the model's logits for the left or right asset. The second three outputs represent the logits deciding among rotation, asset change, or translation. And the last set of logits represent the miner deciding its selection for the chosen category. Given the left/right and the rotation/asset/translation choices, we mask out a subset of these selection logits and renormalize the remaining to be a probability distribution. For example, if the model selects left digit and translation, but the left digit is already at the far left side, then we mask out any translations that would push it beyond the border. We then give it reward based on the cross entropy difference of the resulting perception module's binary prediction \ak{wanna add some more detail here for why not use the model probs i.e. access the model internals? Do we know if access to the prob improves RLMiner?} from the true label and train it with the normal policy gradient update.

% \subsection{Results}

% With all models allowed just a single change, the RandomMiner yields a $1.4\%$ average error for P30, which is within bounds of its own error. The RLMiner gets a $15.0\%$ average error at convergence and the OptimalMiner finds a $33.9\%$ error. \cinjon{Show the results in a graph.} This suggests that a naive policy-gradient RLMiner is capable of finding challenging examples.

% We then use the OptimalMiner for further experiments where we 1) assess how best to finetune P30 with these found examples, 2) ask what a Miner could find after finetuning, and 3) evaluate if the found examples would be applicable to other models.

% \paragraph{What is the best strategy to finetune P30?} We would like to settle on a finetuning strategy that consistently works across mining efforts.

% We refer to the first dataset of mined examples from OptimalMiner as $\textrm{D}_{opt1}$. Recall that these yielded a $34\%$ error rate on P30. We test 21 different settings ranging over two conditions. The first condition is how many mined examples to include out of $[50, 250, 500, 1000, 1500, 2000, 5000]$. The second condition is the ratio of how many examples to include from the original training distribution relative to these out of $[19:1, 9:1, \text{and } 3:1]$. For example, if we select $1000$ examples at a $9:1$ ratio, then we randomly choose the $1000$ mined examples as $\textrm{Opt1}$. \ak{a bit unclear, prolly best to say the 9000 right here?}

% On every epoch of finetuning, we also generate $9000$ examples from the original training distribution, into which we shuffle $\textrm{Opt1}$ to create the finetuning dataset. We then get a score corresponding to the highest attained validation score on a held out set of 8192 mined examples, conditioned on the model still attaining at least the original scores on $\textrm{validation}_1$ and $\textrm{validation}_2$. We do this because we do not want to lose efficacy on the original training set. While we can be losing some subgroup accuracy, we at least ensure that it is correct at the population level. Note however that all of the models do do well on the new mined examples \cinjon{TODO: show that graph}.

% In Fig~\ref{fig:conditional-mined}, we see that for 3:1 \ak{TODO: fix fig and text to be consistent with 0.1 or 1:9?}, where we have only three original examples for every new mined example, for number of examples less than 2000, the model never learns well enough on both validation sets at once. In short, it overindexes. On the other hand, for both 9:1 and 19:1, we see a correlation where roughly the more examples, the better the model does while preserving the original validation score.

% \begin{figure}[!h]
%     \centering
%     \includegraphics[width=7.25cm]{imgs/conditional-mined.png}
%     \caption{TODO}
%     \label{fig:conditional-mined}%
% \end{figure}


% \paragraph{What does the OptimalMiner find in round two?} We would like to know if the model has improved after finetuning. We take a subset of these finetuned models and again ask the OptimalMiner to find where they are weak. 

% The subset we chose corresponds to mined examples in $[250, 2000, 5000]$ and ratios in $[19:1, 9:1, 3:1]$. We further allowed the miner to take two actions instead of one, each time looking for the optimal move, yielding 18 (\ie $3\times3\times2$) new datasets $\textrm{Opt2}, \ldots, \textrm{Opt19}$. Fig~\ref{fig:recycled-absolute} shows how the finetuned models each fair better than the original P30 (\cinjon{TODO, expand analysis}). \ak{we might need more datapoints for the x axis to make sure the 5000 result is not an outlier?} 

% Fig~\ref{fig:recycled-diff} shows the difference of these models versus P30's validation efficacy on the newly mined examples. With too few examples from $\textrm{Opt1}$ included in the finetuning, P30 model does better on the new datasets than the finetuned model. It further appears that there is a threshold past which the model is better off seeing more examples than not. \ak{1 action seems to consistently achieve better diff / higher error than 2 actions at 0.25 data ratio?}


% \begin{figure}[!h]
%     \centering
%     \includegraphics[width=7.25cm]{imgs/recycled-absolute.png}
%     \caption{TODO}
%     \label{fig:recycled-absolute}%
% \end{figure}

% \begin{figure}[!h]
%     \centering
%     \includegraphics[width=7.25cm]{imgs/recycled-diff.png}
%     \caption{TODO}
%     \label{fig:recycled-diff}%
% \end{figure}


% \paragraph{Can the found examples be applicable to other models?} It is rarely the case that we have a single perception module, but rather that we train different ones for different tasks or different organizations. Ideally, we would be able to mine one perception module and have the found hard examples be genuinely difficult for the class of functions that we could learn from the given architecture. 

% Towards answering that, we train six more models, $Q0, \ldots, Q5$, similarly to how we trained P30. We used the same number of epochs, the same architecture, and the same approach to generating the data. The one difference is that we used a different starting seed for creating the distributions. We then evaluated these seven models on the held out test sets of the 19 datasets $Opt[1,19]$, with the x-axis showing the dataset and the y-axis the percent correct. We also show the average of the six Q models as a comparison. 

% We see that sometimes P30 does a lot worse than the others, for example on Opt1 or Opt9. That is the expected though given that this Miner is trying to find very hard examples for that model. However, we also see times where it is among the top models such as in Opt7, Opt10, or Opt13. The common case is that it is on par with the average of the other models. This suggests that the examples mined with P30 are also difficult for an average other model as well.


% \begin{figure*}[!h]
%     \centering
%     \includegraphics[width=\textwidth]{imgs/comparison-models.png}
%     \caption{TODO}
%     \label{fig:comparison-models}%
% \end{figure*}

% \section{Cars}

==> core/unused/8_broader_impact.tex <==

% \section*{Acknowledgements}



